Typosquatting for Fun and Profit: Cross-Country Analysis of Pop-Up Scam

Today, many different types of scams can be found on the internet. Online criminals are always finding new creative ways to trick internet users, be it in the form of lottery scams, downloading scam apps for smartphones or fake gambling websites. This paper presents a large-scale study on one particular delivery method of online scam: pop-up scam on typosquatting domains. Typosquatting describes the concept of registering domains which are very similar to existing ones while deliberately containing common typing errors; these domains are then used to trick online users while under the belief of browsing the intended website. Pop-up scam uses JavaScript alert boxes to present a message which attracts the user's attention very effectively, as they are a blocking user interface element. Our study among typosquatting domains derived from the Majestic Million list utilising an Austrian IP address revealed on 1219 distinct typosquatting URLs a total of 2577 pop-up messages, out of which 1538 were malicious. Approximately a third of those distinct URLs (403) were targeted and displayed pop-up messages to one specific HTTP user agent only. Based on our scans, we present an in-depth analysis as well as a detailed classification of different targeting parameters (user agent and language) which triggered varying kinds of pop-up scams. Furthermore, we expound the differences of current pop-up scam characteristics in comparison with a previous scan performed in late 2018 and examine the use of IDN homograph attacks as well as the application of message localisation using additional scans with IP addresses from the United States and Japan.

==> apk_analysis.tex <==
\subsection{Payload Analysis}
\label{sub:Payload analysis}
This section deals with the payloads behind pop-up scam in the form of mobile apps. Since it is possible to install apps on Android without going through the official distribution channel (Google Play Store), a strong focus on APKs in pop-up scam campaigns is not surprising. In addition to APK files, however, iOS apps (\texttt{*.ipa}) were also found to a small extent. These apps are installed bypassing the official AppStore via company certificates on iOS devices. Almost all payloads can be classified as Trojans.

The app QuVideo for iOS was analyzed in detail to get a deeper understanding of the malware distribution strategies. While the actual binary file of the app is a player for adult videos from mainland China \textcolor{red}{wahlweise auch PR China, aber ich würd da als politisch sensibler Mensch gerne genau sein und nicht Taiwan dissen ;)} and does not contain any signs of malware (as confirmed by VirusTotal \textcolor{red}{Fußnote/Link notwendig?}), a dynamically loadable library (\texttt{libzheng(1).dylib}) contains unambiguous signs of malware that can actually be identified as a variant of TinyV, \textcolor{red}{detto hier, Fußnote/Link/Referenz?} a malware which exploits jailbroken iOS devices.

\textcolor{red}{TODO (Sebastian): mehr Details, ev. noch eine APK?}

==> drafts.tex <==
\section{Drafts - US Scan}
\label{sec:drafts}

\textbf{AT Scan}
\begin{obeylines}
total of $2\,577$ recorded alert boxes
$1\,538$ malicious alert boxes
$303$ distinct messages
$1\,219$ distinct sites
$403$ websites displayed an alert box only to one particular user agent
$816$ websites showed messages to more than one user agent
$102$ distinct messages were only shown to one particular user agent
$201$ to more than one
\end{obeylines}

\textbf{US Scan}
\begin{obeylines}
total of $2\,420$ recorded alert boxes
$1\,393$ malicious alert boxes
$298$ distinct messages
$1\,155$ distinct sites
$382$ websites displayed an alert box only to one particular user agent
$773$ websites showed messages to more than one user agent
$94$ distinct messages were only shown to one particular user agent
$204$ to more than one
\end{obeylines}

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:45]
            unset key
            set xlabel "user agents"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_us/unique_messages_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_us/unique_messages_per_useragent" using 1:($3+2):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages displayed \\ to one particular user agent}
        \label{fig:uniquemessages_us}
        % fig 4
    \end{minipage}
        \hfill
     \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            set yrange [0.1:2500]
            set logscale y
            unset ytics
            unset key
            set xlabel "user agents"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_us/unique_urls_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_us/unique_urls_per_useragent" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of websites targeting one \\ particular user agent}
        \label{fig:uniquesites_us}
        % fig 1
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:150]
            unset key
            set xlabel "categories"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_us/messages_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_us/messages_per_category" using 1:($3+3.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages per category}
        \label{fig:messages_category_us}
        % fig 5
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0.1:15000]
            unset key
            set logscale y
            set xlabel "categories"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_us/sites_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_us/sites_per_category" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct sites per category}
        \label{fig:sites_category_us}
        % fig 6
    \end{minipage}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "25" 25)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:30]
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_us/messages_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different user agents in malicious categories}
     \label{fig:messages_category_useragent_us}
    % fig 9
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set logscale y
        set key left box
        set yrange [0.1:3000]
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        plot 'Data_us/sites_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different user agents in malicious categories}
         \label{fig:sites_category_useragent_us}
        % fig 8
    \end{minipage}
\end{figure*}


\begin{figure}
    \begin{gnuplot}[terminal=pdf,scale=0.6]
        set boxwidth 0.5
        set style fill solid
        unset ytics
        set yrange [0.1:3500]
        unset key
        set xlabel "languages (ISO 639-1)"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        set for [i=1:18] linetype i lc rgb '#d8d8d8'
        set linetype 3 lc rgb '#316ba7'
        set linetype 2 lc rgb '#223b89'
        set linetype 1 lc rgb '#151e5e'
        set linetype 5 lc rgb '#70c3d0'
        set linetype 4 lc rgb '#419dc5'
        plot "Data_us/languages_per_sites" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_us/languages_per_sites" using 1:($3+$3*0.6):3 with labels font "Arial,10"
    \end{gnuplot}
    \caption{Number of distinct sites displaying messages in a specific language}
    \label{fig:languages_sites_us}
    % fig 16
\end{figure}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "30" 30, "50" 50, "60" 60)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:70]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_us/languages_per_unique_messages_per_all_category2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by category}
        \label{fig:languages_categories_us}
        % fig 15
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_us/languages_per_sites_per_category' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by category}
        \label{fig:languages_sites_categories_us}
        % fig 15
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "20" 20, "30" 30, "40" 40, "60" 60, "80" 80)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:120]
        set xlabel "user agents"
        set ylabel "distinct messages"
        plot 'Data_us/languages_per_unique_messages_per_useragent2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by user agent}
        \label{fig:language_messages_useragent_us}
        % fig 11
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
         set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xlabel "user agents"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_us/languages_per_sites_per_useragent' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by user agent}
        \label{fig:language_sites_useragent_us}
        % fig 11
    \end{minipage}
\end{figure*}

\textbf{JP Scan}

\begin{obeylines}
total of $2403$ recorded alert boxes
$1403$ malicious alert boxes
$305$ distinct messages
$1098$ distinct sites
$336$ websites displayed an alert box only to one particular user agent
$762$ websites showed messages to more than one user agent
$103$ distinct messages were only shown to one particular user agent
$202$ to more than one
\end{obeylines}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:45]
            unset key
            set xlabel "user agents"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_jp/unique_messages_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_jp/unique_messages_per_useragent" using 1:($3+2):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages displayed \\ to one particular user agent}
        \label{fig:uniquemessages_jp}
        % fig 4
    \end{minipage}
        \hfill
     \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            set yrange [0.1:2500]
            set logscale y
            unset ytics
            unset key
            set xlabel "user agents"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_jp/unique_urls_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_jp/unique_urls_per_useragent" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of websites targeting one \\ particular user agent}
        \label{fig:uniquesites_jp}
        % fig 1
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:150]
            unset key
            set xlabel "categories"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_jp/messages_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_jp/messages_per_category" using 1:($3+3.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages per category}
        \label{fig:messages_category_jp}
        % fig 5
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0.1:15000]
            unset key
            set logscale y
            set xlabel "categories"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_jp/sites_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_jp/sites_per_category" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct sites per category}
        \label{fig:sites_category_jp}
        % fig 6
    \end{minipage}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "25" 25)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:30]
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_jp/messages_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different user agents in malicious categories}
     \label{fig:messages_category_useragent_jp}
    % fig 9
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set logscale y
        set key left box
        set yrange [0.1:3000]
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        plot 'Data_jp/sites_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different user agents in malicious categories}
         \label{fig:sites_category_useragent_jp}
        % fig 8
    \end{minipage}
\end{figure*}


\begin{figure}
    \begin{gnuplot}[terminal=pdf,scale=0.6]
        set boxwidth 0.5
        set style fill solid
        unset ytics
        set yrange [0.1:3500]
        unset key
        set xlabel "languages (ISO 639-1)"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        set for [i=1:18] linetype i lc rgb '#d8d8d8'
        set linetype 3 lc rgb '#316ba7'
        set linetype 2 lc rgb '#223b89'
        set linetype 1 lc rgb '#151e5e'
        set linetype 5 lc rgb '#70c3d0'
        set linetype 4 lc rgb '#419dc5'
        plot "Data_jp/languages_per_sites" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_jp/languages_per_sites" using 1:($3+$3*0.6):3 with labels font "Arial,10"
    \end{gnuplot}
    \caption{Number of distinct sites displaying messages in a specific language}
    \label{fig:languages_sites_jp}
    % fig 16
\end{figure}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "30" 30, "50" 50, "60" 60)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:70]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_jp/languages_per_unique_messages_per_all_category2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by category}
        \label{fig:languages_categories_jp}
        % fig 15
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_jp/languages_per_sites_per_category' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by category}
        \label{fig:languages_sites_categories_jp}
        % fig 15
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "20" 20, "30" 30, "40" 40, "60" 60, "80" 80)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:120]
        set xlabel "user agents"
        set ylabel "distinct messages"
        plot 'Data_jp/languages_per_unique_messages_per_useragent2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by user agent}
        \label{fig:language_messages_useragent_jp}
        % fig 11
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
         set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xlabel "user agents"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_jp/languages_per_sites_per_useragent' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by user agent}
        \label{fig:language_sites_useragent_jp}
        % fig 11
    \end{minipage}
\end{figure*}


==> plots_jp.tex <==

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:45]
            unset key
            set xlabel "user agents"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_jp/unique_messages_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_jp/unique_messages_per_useragent" using 1:($3+2):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages displayed \\ to one particular user agent}
        \label{fig:uniquemessages_jp}
        % fig 4
    \end{minipage}
        \hfill
     \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            set yrange [0.1:2500]
            set logscale y
            unset ytics
            unset key
            set xlabel "user agents"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_jp/unique_urls_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_jp/unique_urls_per_useragent" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of websites targeting one \\ particular user agent}
        \label{fig:uniquesites_jp}
        % fig 1
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:150]
            unset key
            set xlabel "categories"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_jp/messages_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_jp/messages_per_category" using 1:($3+3.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages per category}
        \label{fig:messages_category_jp}
        % fig 5
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0.1:15000]
            unset key
            set logscale y
            set xlabel "categories"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_jp/sites_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_jp/sites_per_category" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct sites per category}
        \label{fig:sites_category_jp}
        % fig 6
    \end{minipage}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "25" 25)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:30]
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_jp/messages_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different user agents in malicious categories}
     \label{fig:messages_category_useragent_jp}
    % fig 9
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set logscale y
        set key left box
        set yrange [0.1:3000]
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        plot 'Data_jp/sites_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different user agents in malicious categories}
         \label{fig:sites_category_useragent_jp}
        % fig 8
    \end{minipage}
\end{figure*}


\begin{figure}
    \begin{gnuplot}[terminal=pdf,scale=0.6]
        set boxwidth 0.5
        set style fill solid
        unset ytics
        set yrange [0.1:3500]
        unset key
        set xlabel "languages (ISO 639-1)"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        set for [i=1:18] linetype i lc rgb '#d8d8d8'
        set linetype 3 lc rgb '#316ba7'
        set linetype 2 lc rgb '#223b89'
        set linetype 1 lc rgb '#151e5e'
        set linetype 5 lc rgb '#70c3d0'
        set linetype 4 lc rgb '#419dc5'
        plot "Data_jp/languages_per_sites" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_jp/languages_per_sites" using 1:($3+$3*0.6):3 with labels font "Arial,10"
    \end{gnuplot}
    \caption{Number of distinct sites displaying messages in a specific language}
    \label{fig:languages_sites_jp}
    % fig 16
\end{figure}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "30" 30, "50" 50, "60" 60)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:70]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_jp/languages_per_unique_messages_per_all_category2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by category}
        \label{fig:languages_categories_jp}
        % fig 15
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_jp/languages_per_sites_per_category' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by category}
        \label{fig:languages_sites_categories_jp}
        % fig 15
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "20" 20, "30" 30, "40" 40, "60" 60, "80" 80)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:120]
        set xlabel "user agents"
        set ylabel "distinct messages"
        plot 'Data_jp/languages_per_unique_messages_per_useragent2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by user agent}
        \label{fig:language_messages_useragent_jp}
        % fig 11
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
         set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xlabel "user agents"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_jp/languages_per_sites_per_useragent' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by user agent}
        \label{fig:language_sites_useragent_jp}
        % fig 11
    \end{minipage}
\end{figure*}


==> plots_us.tex <==

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:45]
            unset key
            set xlabel "user agents"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_us/unique_messages_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_us/unique_messages_per_useragent" using 1:($3+2):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages displayed \\ to one particular user agent}
        \label{fig:uniquemessages_us}
        % fig 4
    \end{minipage}
        \hfill
     \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            set yrange [0.1:2500]
            set logscale y
            unset ytics
            unset key
            set xlabel "user agents"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#3c1357'
            set linetype 2 lc rgb '#61208d'
            set linetype 3 lc rgb '#a73b8f'
            set linetype 4 lc rgb '#e8638b'
            set linetype 5 lc rgb '#f4aea3'
            plot "Data_us/unique_urls_per_useragent" using 1:3:($0+1):xtic(2) title "unique urls per useragent" with boxes lc variable,"Data_us/unique_urls_per_useragent" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of websites targeting one \\ particular user agent}
        \label{fig:uniquesites_us}
        % fig 1
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0:150]
            unset key
            set xlabel "categories"
            set ylabel "distinct messages"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_us/messages_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_us/messages_per_category" using 1:($3+3.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct messages per category}
        \label{fig:messages_category_us}
        % fig 5
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
            set boxwidth 0.5
            set style fill solid
            unset ytics
            set yrange [0.1:15000]
            unset key
            set logscale y
            set xlabel "categories"
            set ylabel "distinct sites (log_{10} scale)"
            set linetype 1 lc rgb '#54362f'
            set linetype 2 lc rgb '#8a402b'
            set linetype 3 lc rgb '#c04b29'
            set linetype 4 lc rgb '#e45e2d'
            set linetype 5 lc rgb '#e97e3b'
            set linetype 6 lc rgb '#ef9c49'
            set linetype 7 lc rgb '#f5bc59'
            set linetype 8 lc rgb '#fbdc68'
            set linetype 9 lc rgb '#fded82'
            plot "Data_us/sites_per_category" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_us/sites_per_category" using 1:($3+$3*0.6):3 with labels font "Arial,10"
        \end{gnuplot}
        \caption{Number of distinct sites per category}
        \label{fig:sites_category_us}
        % fig 6
    \end{minipage}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "25" 25)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:30]
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_us/messages_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different user agents in malicious categories}
     \label{fig:messages_category_useragent_us}
    % fig 9
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
    
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set logscale y
        set key left box
        set yrange [0.1:3000]
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        plot 'Data_us/sites_per_category_per_useragent' using 2:xtic(1) title col lc rgb '#3c1357', \
                '' using 3:xtic(1) title col lc rgb '#61208d', \
                '' using 4:xtic(1) title col lc rgb '#a73b8f', \
                '' using 5:xtic(1) title col lc rgb '#e8638b', \
                '' using 6:xtic(1) title col lc rgb '#f4aea3'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different user agents in malicious categories}
         \label{fig:sites_category_useragent_us}
        % fig 8
    \end{minipage}
\end{figure*}


\begin{figure}
    \begin{gnuplot}[terminal=pdf,scale=0.6]
        set boxwidth 0.5
        set style fill solid
        unset ytics
        set yrange [0.1:3500]
        unset key
        set xlabel "languages (ISO 639-1)"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        set for [i=1:18] linetype i lc rgb '#d8d8d8'
        set linetype 3 lc rgb '#316ba7'
        set linetype 2 lc rgb '#223b89'
        set linetype 1 lc rgb '#151e5e'
        set linetype 5 lc rgb '#70c3d0'
        set linetype 4 lc rgb '#419dc5'
        plot "Data_us/languages_per_sites" using 1:3:($0+1):xtic(2) with boxes lc variable,"Data_us/languages_per_sites" using 1:($3+$3*0.6):3 with labels font "Arial,10"
    \end{gnuplot}
    \caption{Number of distinct sites displaying messages in a specific language}
    \label{fig:languages_sites_us}
    % fig 16
\end{figure}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "10" 10, "20" 20, "30" 30, "50" 50, "60" 60)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:70]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct messages"
        plot 'Data_us/languages_per_unique_messages_per_all_category2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by category}
        \label{fig:languages_categories_us}
        % fig 15
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xtics rotate by -45
        set xlabel "categories"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_us/languages_per_sites_per_category' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by category}
        \label{fig:languages_sites_categories_us}
        % fig 15
    \end{minipage}
\end{figure*}


\begin{figure*}[!t]
    \centering
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
        set ytics ("5" 5, "20" 20, "30" 30, "40" 40, "60" 60, "80" 80)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0:120]
        set xlabel "user agents"
        set ylabel "distinct messages"
        plot 'Data_us/languages_per_unique_messages_per_useragent2' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct messages over \\ different languages by user agent}
        \label{fig:language_messages_useragent_us}
        % fig 11
    \end{minipage}
    \hfill
    \begin{minipage}[t]{.49\textwidth}
        \begin{gnuplot}[terminal=pdf,scale=0.6]
        set style data histogram
        set style histogram cluster gap 1
         set ytics ("5" 5 ,"10" 10, "50" 50, "100" 100, "500" 500, "800" 800)
        set style fill solid
        set auto x
        set grid ytics
        set key left box
        set yrange [0.1:3000]
        set xlabel "user agents"
        set ylabel "distinct sites (log_{10} scale)"
        set logscale y
        plot 'Data_us/languages_per_sites_per_useragent' using 2:xtic(1) title col lc rgb '#151e5e', \
                '' using 3:xtic(1) title col lc rgb '#223b89', \
                '' using 4:xtic(1) title col lc rgb '#316ba7', \
                '' using 5:xtic(1) title col lc rgb '#419dc5', \
                '' using 6:xtic(1) title col lc rgb '#70c3d0', \
                '' using 7:xtic(1) title col lc rgb '#d8d8d8'
        \end{gnuplot}
        \caption{Distribution of distinct sites over \\ different languages by user agent}
        \label{fig:language_sites_useragent_us}
        % fig 11
    \end{minipage}
\end{figure*}
